Smooth Attention for Deep Multiple Instance Learning: Application to CT Intracranial Hemorrhage Detection

Multiple Instance Learning (MIL) has been widely applied to medical imaging diagnosis, where bag labels are known and instance labels inside bags are unknown. Traditional MIL assumes that instances in each bag are independent samples from a given distribution. However, instances are often spatially or sequentially ordered, and one would expect similar diagnostic importance for neighboring instances. To address this, in this study, we propose a smooth attention deep MIL (SA-DMIL) model. Smoothness is achieved by the introduction of first and second order constraints on the latent function encoding the attention paid to each instance in a bag. The method is applied to the detection of intracranial hemorrhage (ICH) on head CT scans. The results show that this novel SA-DMIL: (a) achieves better performance than the non-smooth attention MIL at both scan (bag) and slice (instance) levels; (b) learns spatial dependencies between slices; and (c) outperforms current state-of-the-art MIL methods on the same ICH test set.

==> MICCAI.tex <==
{\color{red}
==============I'M MODIFYING THIS =======}

As described in the original paper, sparse Gaussian processes ($SGP$) are applied to predict the instance probabilities:
\begin{equation} \label{eq_sgp}
     p(y_{bi}|z_{bi}) = SGP(z_{bi})
\end{equation}
The probability of the bag label is described by a differentiable function which approximates the max-function and is necessary for the optimization. We obtain the bag prediction by:
\begin{equation} \label{eq_max_agg}
     p(Y_b|\{y_{b1},.., y_{bI_b}\}) = \frac{H^{G_b}}{H+1}
\end{equation}
where $G_b = Y_b \max_i\{y_{bi}\} + (1 - Y_b)(1 - \max_i\{y_{bi}\})$ and $H$ is a constant that defines the level of approximation to the max function: the higher $H$, the closer the approximation. As the true posterior $P(Y|X)$ in this context is intractable, a variational distribution $Q(Y|X)$ is used which is optimized by minimizing the Kullback-Leibler divergence:
\begin{equation}
    \underset{Q}{\mathrm{argmin}} \ KL(Q(Y|X)||P(Y|X)) 
\end{equation}
The optimization is done using the evidence lower bound (ELBO) and the mean field method. For further details we refer to the original paper \cite{ilse_attention-based_2018,shen_doubly_2019}.

For testing, the $f_{cnn}$ is used to extract the features and the VGPMIL model to obtain instance and bag predictions.

{\color{red}
======================UNTIL HERE ======}
